Lexical Generalization Improves with Larger Models and Longer Training

While fine-tuned language models perform well on many tasks, they were also shown to rely on superficial surface features such as lexical overlap. Excessive utilization of such heuristics can lead to failure on challenging inputs. We analyze the use of lexical overlap heuristics in natural language inference, paraphrase detection, and reading comprehension (using a novel contrastive dataset), and find that larger models are much less susceptible to adopting lexical overlap heuristics. We also find that longer training leads models to abandon lexical overlap heuristics. Finally, we provide evidence that the disparity between models size has its source in the pre-trained model

==> tables/alsqa_results.tex <==

% \begin{table}
% \centering
% % \resizebox{1\columnwidth}{!}{%
% \begin{tabular}{llllll}
% \hline
% \multicolumn{5}{c}{RoBERTa base}  \\
% \hline
% \multicolumn{2}{c}{} & \multicolumn{2}{c}{EM}  & \multicolumn{2}{c}{F1}  \\
% \hline
% \textbf{Dataset} & & first & final & first & first  \\
% \hline
% % ALSQA & Low    &70.8 	 & 73.5  & 70.8 &73.9\\
% %       & Medium &72.5 	 & 75.5  & 73.7 &77.4\\
% %       & High   &76.2 	 & 78.7  & 76.2 &79.7\\
% ALSQA & Low    &70.8 	 & 70.8  &  73.5 &73.9\\
%       & Medium &72.5 	 &73.7  & 75.5 &77.4\\
%       & High   &76.2 	 & 76.2  & 78.7 &79.7\\
% \hline
% SQuAD & Dev &78.1 	 & 81.4  & 79.0 &82.6\\

% \end{tabular}


% \begin{tabular}{llllll}
% \hline
% \multicolumn{5}{c}{RoBERTa large}  \\
% \hline
% \multicolumn{2}{c}{} & \multicolumn{2}{c}{EM}  & \multicolumn{2}{c}{F1}  \\
% \hline
% \textbf{Dataset} & & first & final & first & final  \\
% \hline
% % ALSQA & Low    &76.3 	 & 79.0  & 78.5 &81.7\\
% %       & Medium &77.9 	 & 80.7  & 80.5 &83.7\\
% %       & High   &80.8	 & 83.6  & 80.4 &83.9\\

% ALSQA & Low    &76.3 	 & 78.5  & 79.0 &81.7\\
%       & Medium &77.9 	 & 80.5  & 80.7 &83.7\\
%       & High   &80.8	 & 80.4  & 83.6 &83.9\\
% \hline
% SQuAD & Dev &83.0 	 & 85.9  & 83.6 & 87.2\\

% \end{tabular}
% % }
% \caption{
% The results on ALSQA
% }

% \label{tab:alsqa_res}
% \end{table}



%%%%%%%%%%%%%


\begin{table}
\centering
\resizebox{1\columnwidth}{!}{%


\begin{tabular}{llrrrrr}
\hline

Version & Model & Dev & Low & Medium & High & HEUR \\
\hline

first & base  & 78.1/81.4 & 70.8/73.5 & 72.5/75.5 & 76.2/79.7 & 3.6/3.5 \\
      & large & 83.0/85.9 & 76.3/79.0 & 77.9/80.7 & 80.8/83.6 & 3.0/3.0 \\
\hline
last & base   & 79.0/82.6        & 70.8/73.9 & 73.7/77.4 & 76.2/79.7 & 3.6/3.9 \\
     & large  & 83.6/87.2        & 78.5/81.7 & 80.5/83.7 & 80.4/83.9 & 1.3/1.5 \\

\end{tabular}
}
\caption{
The results on ALSQA (Yanai's proposal). can also report only F1 or EM, and the full results to be added to the appendix. Also, make sure that the dev results are on the first epoch, and not last, and fill up the other
EM/F1.
}
\vspace{-6mm}
\label{tab:alsqa_res}
\end{table}

==> tables/alsqa_stats.tex <==
\begin{table}
\centering
\begin{tabular}{l|lll|l}
\hline
\textbf{Overlap} & \textbf{Has} & \textbf{No}  &\textbf{Total}&\textbf{Mean}\\
\textbf{Class} & \textbf{Ans} & \textbf{Ans}  & &\textbf{Overlap}\\
\hline
\hline
High & 371 & 370 & 741 & 0.98\\
Medium &371 & 370 & 741 & 0.67 \\
Low &371 & 370 & 741 & 0.21 \\
\hline
Total &1113 & 1110 & 2223  \\
\end{tabular}
\caption{Number of examples with and without answer at every overlap class of ALSQA and the mean overlap coefficient at every class.}
\label{tab:alsqa_count}
\end{table}

==> tables/dev_results.tex <==
\begin{table}
\centering
\begin{tabular}{lcccc}
\hline
\textbf{Dataset} & \textbf{Model}& \textbf{Median}& \textbf{Max}\\
\hline
MNLI &  RoBERTa (base)  & 87.1 & 87.6 \\
(Acc) &  RoBERTa (large)  & 89.3 & 89.8 \\
\hline
QQP &  RoBERTa (base)  & 91.6 & 91.7 \\
(Acc) &  RoBERTa (large)  & 91.9 & 92.1 \\
 \hline
 SQuAD2 &  RoBERTa (base) & 82.6 & 83.6 \\
(F1) &  RoBERTa (large)  & 87.2 & 88.2 \\

\end{tabular}
\caption{The development set median results of the RoBERTa models we finetuned.}
\label{tab:dev_res}
\end{table}
